Kernel Methods and their derivatives: Concept and perspectives for the Earth system sciences

Kernel methods are powerful machine learning techniques which implement generic non-linear functions to solve complex tasks in a simple way. They Have a solid mathematical background and exhibit excellent performance in practice. However, kernel machines are still considered black-box models as the feature mapping is not directly accessible and difficult to interpret.The aim of this work is to show that it is indeed possible to interpret the functions learned by various kernel methods is intuitive despite their complexity. Specifically, we show that derivatives of these functions have a simple mathematical formulation, are easy to compute, and can be applied to many different problems. We note that model function derivatives in kernel machines is proportional to the kernel function derivative. We provide the explicit analytic form of the first and second derivatives of the most common kernel functions with regard to the inputs as well as generic formulas to compute higher order derivatives. We use them to analyze the most used supervised and unsupervised kernel learning methods: Gaussian Processes for regression, Support Vector Machines for classification, Kernel Entropy Component Analysis for density estimation, and the Hilbert-Schmidt Independence Criterion for estimating the dependency between random variables. For all cases we expressed the derivative of the learned function as a linear combination of the kernel function derivative. Moreover we provide intuitive explanations through illustrative toy examples and show how to improve the interpretation of real applications in the context of spatiotemporal Earth system data cubes. This work reflects on the observation that function derivatives may play a crucial role in kernel methods analysis and understanding.

==> sections/definitions_v2.tex <==
\renewcommand{\sectionautorefname}{\S}
\newcommand{\Real}{{\mathbb R}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\muno}{\mbox{\sf\scriptsize-1}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}

\newcommand{\bk}{\mathbf{k}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\n}{\mathbf{n}}
\newcommand{\w}{{\boldsymbol{\omega}}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}

\newcommand{\prob}{p}

\newcommand{\GP}{{\mathcal G}{\mathcal P}}
\newcommand{\dataset}{{\mathcal D}}
\newcommand{\Normal}[0]{\mathcal{N}}


%%%% LFM


\newcommand{\red}[1]{\textcolor [rgb]{0.5,0,0}{#1}}
\newcommand{\mse}{\textrm{MSE}}
\newcommand{\rmse}{\textrm{NMSE}}
\newcommand{\lai}{\textrm{LAI}}
\newcommand{\fapar}{\textrm{FAPAR}}
\newcommand{\thetavec}{\boldsymbol{\theta}}
\newcommand{\muvec}{\boldsymbol{\mu}}
\newcommand{\Esp}[1]{\textnormal{E}\{#1\}}
\newcommand{\BEsp}[1]{\textnormal{E}\left\{#1\right\}}
\newcommand{\Rbf}{\textnormal{\tiny{RBF}}}
\newcommand{\Wgn}{\textnormal{\tiny{WGN}}}
\newcommand{\diff}{\textnormal{d}}
\newcommand{\linOpGeneral}[4]{\textrm{L}_{#1,#2}[#3]\left\{#4\right\}}
\newcommand{\linOpSpecific}[3]{\textrm{L}_{#1}[#2]\left\{#3\right\}}
\newcommand{\linOpModelSpecific}[4]{\textrm{L}_{#1}^{#2}[#3]\left\{#4\right\}}
\newcommand{\Var}[1]{\textnormal{Var}\{#1\}}

\newcommand{\Erf}[1]{\textnormal{erf}\left(#1\right)}

\newcommand{\map}{\textnormal{MAP}}

\renewcommand{\vec}[1]{\mathbf{#1}}



==> sections/dependence_old_.tex <==
\subsection{Dependence estimation with kernel methods}

Measuring dependencies (nonlinear association) between random variables is an active field of research. The principle underlying kernel-based dependence estimation is that it allows one to define covariance and cross-covariance operators in RKHS, and derive statistics from these operators capable of measuring dependence between functions therein. %A wide variety of empirical kernel dependence estimates has been proposed. Not long ago, in ~\cite{BacJor02}, a regularized correlation operator was derived from the covariance and cross-covariance operators and its largest singular value (the kernel canonical correlation, or KCC) was used as a statistic to test independence. Later in~\cite{GreSmoBouHeretal05}, the largest singular value of the cross-covariance operator was proposed as an efficient alternative that needs no regularization. This test is called the constrained covariance (COCO)~\cite{GreSmoBouHeretal05}. Other quantities have been derived from bounds on the mutual information that hold near independence, such as the kernel Generalised Variance (kGV) and the Kernel Mutual Information (kMI)~\cite{GreHerSmo03,Gretton05}. 
Among the most interesting developments, we find the Hilbert-Schmidt Independence Criterion (HSIC)~\cite{GreBouSmoSch05}. The method consists of measuring cross-covariances in a proper RKHS. %, and extends previous methods by using the entire spectrum of the cross-covariance operator, not just the largest singular value. 

Notationally, let us consider two spaces ${\mathcal X}\subseteq \Real^{d_x}$ and ${\mathcal Y}\subseteq \Real^{d_y}$, on which we jointly sample observation pairs $(\x,\y)$ from distribution ${\mathbb P}_{\x\y}$. The covariance matrix is ${\mathcal C}_{\x\y} = {\mathbb E}_{\x\y}(\x\y^\top) - {\mathbb E}_{\x}(\x){\mathbb E}_{\y}(\y^\top)$, where ${\mathbb E}_{\x\y}$ is the expectation with respect to ${\mathbb P}_{\x\y}$, ${\mathbb E}_{\x}$ is the expectation with respect to the marginal distribution ${\mathbb P}_{\x}$ (here and below, we assume that all these quantities exist), and $\y^\top$ is the transpose of $\y$. The covariance matrix encodes all first order dependencies between the random variables. A statistic that efficiently summarizes the content of this matrix is its Hilbert-Schmidt norm. %The square of this norm is equivalent to the squared sum of its eigenvalues $\gamma_i$, $\|{\mathcal C}_{\x\y}\|_{\text{HS}}^2 = \sum_i \gamma_i^2$. 
This quantity is zero if and only if there exists no first order dependence between $\x$  and $\y$. Note that the Hilbert Schmidt norm is limited to the detection of first order relations, and thus more complex (higher-order effects) cannot be captured. 

The nonlinear extension of the notion of covariance was proposed in \cite{GreBouSmoSch05}. Essentially, let us define a (possibly non-linear) mapping $\boldsymbol{\phi}: {\mathcal X}\to {\mathcal F}$  such that the inner product between features is given by a positive definite (p.d.) kernel function  $k_x(\x,\x') = \langle \boldsymbol{\phi}(\x),\boldsymbol {\phi}(\x')\rangle$. The feature space ${\mathcal F}$ has the structure of a reproducing kernel Hilbert space (RKHS). Let us now denote another feature map $\boldsymbol{\psi}:{\mathcal Y}\to {\mathcal G}$ with associated p.d. kernel function {$k_y(\y,\y') = \langle \boldsymbol{\psi}(\y),\boldsymbol{\psi}(\y')\rangle$}. Then, it is possible to define a cross covariance operator between these feature maps, and to compute the squared norm of the cross-covariance operator, $\|{\mathcal C}_{\x\y}\|^2_{\text{HS}}$, which is called the Hilbert-Schmidt Independence Criterion (HSIC) and can be expressed in terms of kernels~\cite{Baker73,Fukumizu04}. Given a sample dataset $Z=\{(\x_1,\y_1),\ldots,(\x_m,\y_m)\}$ of size $m$ drawn from ${\mathbb P}_{\x\y}$, an empirical estimator of HSIC proposed in \cite{GreBouSmoSch05} is:
\begin{eqnarray}
\text{HSIC}({\mathcal F},{\mathcal G},{\mathbb P}_{\x\y}) = 
\dfrac{1}{m^2} \text{Tr}({\bf K}_x{\bf H}{\bf K}_y{\bf H})= 
\dfrac{1}{m^2} \text{Tr}({\bf H}{\bf K}_x{\bf H}~{\bf K}_y),\label{empHSIC}
\end{eqnarray}
where $\text{Tr}(\cdot)$ is the trace operation (the sum of the diagonal entries),  ${\bf K}_x$, ${\bf K}_y$ are the kernel matrices for the input random variables $\x$ and $\y$, respectively, and ${\bf H}= {\bf I} - \frac{1}{n}\mathbbm{1}\mathbbm{1}^\top$ centers the data in the feature spaces ${\mathcal F}$ and ${\mathcal G}$, respectively. HSIC has demonstrated excellent capabilities to detect dependence between random variables but, as for any kernel method, the learned relations are hidden behind the kernel feature mapping. Visualization and geometrical interpretation of kernel methods in general and kernel dependence estimates in particular is an important issue in machine learning. To address this issue, we consider the derivatives of HSIC.

\subsection{Derivatives of HSIC}

The definition of derivative for discriminative kernels is limited in some aspects: 1) it cannot be directly applied to general functions $f$ depending on matrices or tensors, and 2) it allows estimating feature relevances $s_j$ only, discarding the individual samples relevance. The former is a severe limitation in particular for HSIC as it directly deals with data matrices. The latter limitation affects all type of functions including HSIC, which could be useful in applications on outlier detection or sample selection, just to name a few. We take the HSIC derivative~\cite{SHSIC2017}, with respect to the input samples and features simultaneously to address both shortcomings. 

Let us now define $f:=\text{HSIC}$, and replace the derivatives $\frac{\partial f(\param)}{\partial z_j}$ with $\frac{\partial f(\Param)}{\partial Z_{ij}}$. Note that point-wise HSIC is parametrized by $\param\sim \x,\y$, while a matrix parametrization reduces to $\Param\sim{\bf X},{\bf Y}$. In order to compute the HSIC derivatives, and hence their summarizing (sensitivity) maps, we derive HSIC w.r.t. input data matrix entries $X_{ij}$ and $Y_{ij}$. By applying the chain rule, and first-order derivatives of matrices, it is obtained~\cite{Perez17shsic}:
\begin{equation}\label{shsic_x}
%S_{ij}^x:=\dfrac{\partial\text{HSIC}}{\partial X_{ij}}=-\frac{2}{\sigma^2 n^2}\text{Tr}\left({\bf H}{\bf K}_y{\bf H}({\bf K}_x\circ {\bf M}_{ik}^j)\right),
\partial_{ij}^x:=\dfrac{\partial\text{HSIC}}{\partial X_{ij}}=-\frac{2}{\sigma^2 n^2}\text{Tr}\left({\bf H}{\bf K}_y{\bf H}({\bf K}_x\circ {\bf M}_j\right),
\end{equation} 
where for a given $j$th feature, entries of the corresponding matrix ${\bf M}_j$ are $M_{ik}=X_{ij}-X_{kj}$ ($1\leq i,k\leq n$), and the symbol $\circ$ is the Hadamard product between matrices. After operating similarly for $Y_{ij}$, we obtain the corresponding expression:
\begin{equation}\label{shsic_y}
\partial_{ij}^y:=\dfrac{\partial\text{HSIC}}{\partial Y_{ij}} = -\frac{2}{\sigma^2 n^2}\text{Tr}\left({\bf H}{\bf K}_x{\bf H}({\bf K}_y\circ {\bf N}_j)\right),
\end{equation}
where entries of matrix ${\bf N}_j$ are $N_{ik}=Y_{ij}-Y_{kj}$, and we assumed the SE kernel for both variables\footnote{Other positive definite universal kernels could be equally adopted, but that requires deriving the sensitivity maps for the specific kernel.}. 

It is worth noting that, even though one could be tempted to use each derivative map independently, the solution is a {\em vector field}, and we should treat them jointly. % To do this we define the {\em total derivative map} for all features and samples as ${\bf S}:=[{\bf S}^x,{\bf S}^y]\in\Real^{n\times (d_x+d_y)}$. From ${\bf S}$ we can compute the {\em empirical sensitivity map} per either feature or sample by integration in the corresponding domain, whose empirical estimates are respectively 
%$s_i\approx\frac{1}{d}\sum_{j=1}^d S_{ij}^2$ and $s_j\approx\frac{1}{n}\sum_{i=1}^n S_{ij}^2.$
The derivatives of HSIC report information about the directions most impacting the dependence estimate, and allow a quantitive geometric evaluation of the measure. Note that, as in the previous kernel methods, the derivatives here are also analytical, just involving simple matrix multiplications and a trace operation.

\subsection{Visualizing kernel dependence measures} 

Figure~\ref{fig:1_HSIC} shows the directional derivative maps for three different bidimensional problems of variable association. We show the different components of the (sign-valued) vector field, $\partial_x$ and $\partial_y$, as well as its magnitude, $\|[\partial_x,\partial_y]\|$. In all problems, arrows indicate the strength of distortion to be applied to points (either in directions $x$, $y$, or jointly) such that the dependence is maximized. For the first example, the map tries to push points towards the 1-1 line, while on the second case dependence is maximized by trying to cluster the data distribution in a sort of X-OR gate shaped distribution. %It can be noted that low sensitivity values are commonly related to conditional means in Gaussian associations (top row), extremes, joints and change/elbow points in nonlinearly related variables, and clustered/randomly located points in near independence cases.

\begin{figure}[t!]
\begin{center}
\begin{tabular}{ccc}
$\partial_x$ & $\partial_y$  & $\|[\partial_x,\partial_y]\|$ \\
\includegraphics[width=.32\textwidth]{images/experiments/moved/Sx_2.pdf}  &  
\includegraphics[width=.32\textwidth]{images/experiments/moved/Sy_2.pdf}  &  
\includegraphics[width=.32\textwidth]{images/experiments/moved/Sxy_2.pdf}  \\
\includegraphics[width=.32\textwidth]{images/experiments/moved/Sx_20.pdf}  &  
\includegraphics[width=.32\textwidth]{images/experiments/moved/Sy_20.pdf}  &  
\includegraphics[width=.32\textwidth]{images/experiments/moved/Sxy_20.pdf} \\
\includegraphics[width=.32\textwidth]{images/experiments/moved/Sx_16.pdf} &
\includegraphics[width=.32\textwidth]{images/experiments/moved/Sy_16.pdf} &
\includegraphics[width=.32\textwidth]{images/experiments/moved/Sxy_16.pdf}
\end{tabular}
\caption{Visualizing the derivatives for HSIC in three toy examples (Gaussian distributed, circle, and rotated square). We show in arrows the directional derivatives, and in colors their intensity (norm of the pointwise derivative). \red{ADRIAN, REDO IMAGES FOR CLARITY, AND REMOVE THE BOUNDING BOX!}}
\label{fig:1_HSIC}
\end{center}
\end{figure}


%%% \begin{figure}[t!]
%%% \begin{center}
%%% \setlength{\tabcolsep}{-1pt}
%%% \begin{tabular}{ccccccc}
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_1.pdf} &
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_2.pdf} & 
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_3.pdf} &
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_4.pdf} &
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_5.pdf} &
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_6.pdf} &
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_7.pdf} \\
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_15.pdf} &
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_16.pdf} &
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_17.pdf} &
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_18.pdf} &
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_19.pdf} &
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_20.pdf} &
%%% \includegraphics[width=1.8cm]{images/experiments/bivariate_21.pdf} \\
%%% \end{tabular}
%%% \vspace{-0.25cm}
%%% \caption{Results for dependence estimation in 14 toy examples. Each table gives Pearson, Kendall, Spearman (top, left-to-right) and mutual information, and HSIC. We highlight the sensitivity norm per example, where lighter reddish means higher sensitivity.\label{fig:1}}
%%% \end{center}
%%% \end{figure}
\iffalse
\begin{figure}[t!]
\begin{center}
\setlength{\tabcolsep}{-15pt}
\begin{tabular}{ccc}
$S_x$ & $S_y$ & $|S|=\sqrt{S_x^2+S_y^2}$ \\
\includegraphics[width=.32\textwidth]{images/experiments/Sx_2.pdf} &
\includegraphics[width=.32\textwidth]{images/experiments/Sy_2.pdf} & 
\includegraphics[width=.32\textwidth]{images/experiments/Sxy_2.pdf} 
\\
\includegraphics[width=.32\textwidth]{images/experiments/Sx_20.pdf} &
\includegraphics[width=.32\textwidth]{images/experiments/Sy_20.pdf} &
\includegraphics[width=.32\textwidth]{images/experiments/Sxy_20.pdf}
\\
\includegraphics[width=.32\textwidth]{images/experiments/Sx_16.pdf} &
\includegraphics[width=.32\textwidth]{images/experiments/Sy_16.pdf} &
\includegraphics[width=.32\textwidth]{images/experiments/Sxy_16.pdf}
\end{tabular}
\vspace{-0.25cm}
\caption{Visualizing the derivatives and the modulus of the directional derivative for HSIC in three toy examples.} 
\label{fig:1_HSIC}
\end{center}
\end{figure}
\fi



\subsection{Unfolding and Independization}


\begin{figure}[h!]
\centerline{\includegraphics[width=7cm]{./images/composite.pdf}}
\vspace{-0.15cm}
\caption{HSIC dependence maps used to maximize or minimize dependence.}
\label{fig:sensitivity2}
\end{figure}
 
We have seen that the derivatives of the HSIC function can be useful to learn about the data distribution and the variable associations. The derivatives of HSIC give information about the directions most affecting the dependence or independence measure. Figure~\ref{fig:sensitivity2} shows the use of sensitivity to achieve (in)dependence by `moving' samples towards the most (in)sensitive directions in feature space. We embedded the derivatives in a simple gradient descent scheme, in which we move samples iteratively as follows: $\Param{(t+1)}$ = $\Param{(t)}$ $\pm$ $\eta\nabla_{\param}\text{HSIC}(t)$, % = $\X{(t)}\pm\eta~{\bf S}^2_{\x}{(t)},$ and similarly for $\Y$, 
%$$\y_i^j(t+1) = \y_i^j(t)\pm\eta\nabla_{\y_i^j}\text{HSIC}(\x,\y,t) = \y_i^j(t)\pm\eta~\s_{i,j}^y(t),$$
where the sign will lead to maximize or minimize data dependence. Departing from a sinusoide, one can easily attain dependent or independent domains. %unfolded or Gaussinized/uniformized domains, respectively.

\iffalse
\paragraph{Denoising data.} 
Given a noisy observation $\y=f(\x)+{\bf n}$, the aim is to retrieve a good estimation of the noise $\hat n$. We followed an iterative procedure inspired in seeking for maximal dependence between $\x$ and $\y$ through HSIC, in the sense that enforcing this dependence directly remove the noise effect. Then, for iteration $t=1,\ldots,T$, we perform a gradient descent on the sensitivity of HSIC to maximize the dependence with the unknown $f(\x)$. That is,
$$\hat{\y}{(t+1)} = \hat{\y}{(t)} + \eta~\nabla_\y\text{HSIC}(\x,\hat{\y}{(t)}) = \hat{\y} + \eta~{\bf S}_\y^2(\x,\hat{\y}{(t)}),$$
where $\eta>0$ is the learning rate in the gradient descent, and we assume that the noise is only present in the $\y$ direction (otherwise we could use $\nabla_x\text{HSIC}$ as well). After some iterations, we obtain a denoised version of the noisy observation, as shown in Figure~\ref{fig:noise}[top row] for both homoscedastic and heteroscedastic noise and linear and nonlinear functions $f$. In Figure~\ref{fig:noise}[bottom row] we show the cdf of both the original $n$ and the estimated noise $\hat{\bf n}$. This experiment shows how sensitivity maps can be used as the direction which maximizes the dependence between variables leading to intuitively more noise-free distributions. We illustrated this good empirical behavior with different noisy problems.

\begin{figure}[t!]
\begin{center}
\mbox{\includegraphics[width=.25\textwidth]{images/denoising/estim_lin_homo.pdf}
\includegraphics[width=.25\textwidth]{images/denoising/estim_lin_hetero.pdf}
\includegraphics[width=.25\textwidth]{images/denoising/estim_nonlin_homo.pdf}
\includegraphics[width=.25\textwidth]{images/denoising/estim_nonlin_hetero.pdf}}
\\
\mbox{\includegraphics[width=.25\textwidth]{images/denoising/cdf_lin_homo.pdf}
\includegraphics[width=.25\textwidth]{images/denoising/cdf_lin_hetero.pdf}
\includegraphics[width=.25\textwidth]{images/denoising/cdf_nonlin_homo.pdf}
\includegraphics[width=.25\textwidth]{images/denoising/cdf_nonlin_hetero.pdf}}
\end{center}
\vspace{-0.25cm}
\caption{From left to right linear-homo, linear-hetero, nonlinear-homo and nonlinear-heteroscedastic noise problems. Top row shows examples of original observations (black) and denoised signal (blue) for different noise sources, while the bottom row shows their cumulative distribution functions.}\label{fig:noise}
\end{figure}
%%% \begin{figure}[t!]
%%% \centering
%%% \includegraphics[width=.15\textwidth]{./images/experiments/maximize_problem.pdf}
%%% \includegraphics[width=.15\textwidth]{./images/experiments/maximize_min.pdf}
%%% \includegraphics[width=.15\textwidth]{./images/experiments/maximize_max.pdf}\\
%%% \includegraphics[clip=true, trim={1.5cm 1.5cm 1.5cm 1.5cm }, width=.15\textwidth]{./images/experiments/maximize_legend.pdf}
%%% \includegraphics[width=.15\textwidth]{./images/experiments/maximize_min_crits.pdf}
%%% \includegraphics[width=.15\textwidth]{./images/experiments/maximize_max_crits.pdf}
%%% \caption{HSIC sensitivity maps used to maximize/minimize dependence.}
%%% \label{fig:sensitivity_maxmin1}
%%% \end{figure}

%\subsection{Classification with HSIC}


%\begin{figure}[t!]
%\centering
%\includegraphics[width=.3\textwidth]{./images/experiments/origData_1.pdf}
%\includegraphics[width=.3\textwidth]{./images/experiments/transSens_1.pdf}
%\includegraphics[width=.3\textwidth]{./images/experiments/accSens_1.pdf}\\
%\includegraphics[width=.3\textwidth]{./images/experiments/origData_2.pdf}
%\includegraphics[width=.3\textwidth]{./images/experiments/transSens_2.pdf}
%\includegraphics[width=.3\textwidth]{./images/experiments/accSens_2.pdf}\\
%\includegraphics[width=.3\textwidth]{./images/experiments/origData_3.pdf}
%\includegraphics[width=.3\textwidth]{./images/experiments/transSens_3.pdf}
%\includegraphics[width=.3\textwidth]{./images/experiments/accSens_3.pdf}\\
%\caption{HSIC sensitivity maps used to maximize/minimize dependence.}
%\label{fig:sensitivity_maxmin2}
%\end{figure}

\fi




==> sections/derivatives_.tex <==
\subsection*{Summarizing derivative information}
\subsection*{Derivatives of two variables kernel methods}
\subsection*{On the $n$-th order derivatives}



==> sections/kernels.tex <==
Kernel methods rely on the properties of kernel functions. As we will see next, they reduce to compute dot products of vectors mapped in Hilbert spaces through an implicit (not necessarily known) mapping function. A scalar product space (or pre-Hilbert space) is a space endorsed with a scalar product. If the space is {\em complete} (i.e. every Cauchy sequence converges inside the space), then it is called a {\em Hilbert space}. This section conveys a short introduction to kernel methods, functions approximation, and RKHS. The tools reviewed here are of fundamental relevance for the next sections, and build upon solid branches of mathematics such as {\em linear algebra}~\cite{Golub96} and {\em functional analysis}~\cite{ReedSimon81}.

% ###############################################
\subsection{Measuring Similarity with Kernels}
% ###############################################

The dot (scalar or inner) product between two vectors is an algebraic operation that measures the similarity between them. Intuitively, a dot, scalar product measures how much of a vector is contained in the other, or alternatively how much the two vectors point in the same direction. The question raised here is whether one should naively rely on the dot product in the input space to measure the similarity of (possibly complex) objects or not. If the representation space of those objects is rich enough, a dot product in input space should suffice. Unfortunately, many times the input feature space is limited in resolution and expressive power and a new richer representation is needed. Kernel methods rely on the notion of similarity between examples in a higher (possibly infinite dimensional) Hilbert space. Be a set of empirical data $(\bx_1,y_1),\ldots,(\bx_n,y_n)\in\mcalX\times\mcalY$, in which $\bx_i$ are the \emph{inputs} taken from $\mcalX$ and $y_i\in\mcalY$ are called the \emph{outputs}. The learning from samples process  consists of using these data pairs to predict a new set of  test examples $\bx\in\mcalX$. In order to develop learning machines capable of generalizing well, kernel methods often support a good approximation to the structure of the data and incorporate regularization in a natural way.

In some of those cases when  $\mcalX$ does not stand for a good support of similarity, examples can be mapped to a (dot product) space $\mcalH$\index{feature space}, by using a mapping $\bphi:\mcalX\rightarrow\mcalH, \bx\mapsto \bphi(\bx)$. The mapping function can be defined explicitly (if some prior knowledge about the problem is available) or implicitly as in the case of kernel methods. The similarity between the elements in $\mcalH$ can now be measured using its associated dot product $\langle\cdot,\cdot\rangle_{\mcalH}$. Here, we define a function that computes that similarity \index{kernel}, $K:\mcalX\times\mcalX\rightarrow\mathbb{R}$, such that $(\bx,\bx')\mapsto K(\bx,\bx')$. This function, often called \emph{kernel}, is required to satisfy:
\begin{equation}\label{eq:kernel}
  K(\bx,\bx') = \langle \bphi(\bx), \bphi (\bx') \rangle_{\mcalH}.
\end{equation}
The mapping $ \bphi$ is its \emph{feature map}, the space $\mcalH$ is the reproducing Hilbert \emph{feature space}, and $K$ is the reproducing kernel function since it {\em reproduces} dot products in $\mcalH$ without even mapping data explicitly therein.



% ###############################################
\subsection{Positive Definite Kernels}
% ###############################################

The type of kernels that can be written in the form of Eq.~\eqref{eq:kernel} coincides with the class of {\em positive definite kernels}\index{kernel!positive definite}. The property of positive definiteness is crucial in the field of kernel methods.

\begin{definition}\label{prop:existHilbert}
A function $K:\mcalX\times\mcalX\rightarrow\mathbb{R}$ is a positive definite kernel \emph{if and only if} there exists a Hilbert space $\mcalH$ and a feature map $\bphi:\mcalX\rightarrow\mcalH$ such that for all $\bx,\bx' \in\mcalX$, we have $K(\bx,\bx')=\langle \bphi (\bx), \bphi  (\bx')\rangle_{\mcalH}$  for some inner-product space ${\mcalH}$ such that $\forall \bx\in\mcalX$ and $ \bphi \in\mcalH$.
\end{definition}

\begin{definition}\label{prop:kernelmatrix}
A kernel matrix (or Gram matrix) $\bK$ is the matrix that results from applying the kernel function $K$ to all pairs of points in the set $\{\bx_i\}_{i=1}^N$, i.e.,
\begin{equation}
\bK  = \left( \begin{array}{cccc}
K(\bx_1,\bx_1) & K(\bx_1,\bx_2) & \cdots & K(\bx_1,\bx_N)\\
K(\bx_2,\bx_1) & K(\bx_2,\bx_2) & \cdots & K(\bx_2,\bx_N)\\
\vdots & \vdots & \ddots & \vdots\\
K(\bx_N,\bx_1) & K(\bx_N,\bx_2) & \cdots & K(\bx_N,\bx_N) \end{array}\right),
\end{equation}
and whose entries are denoted as $\bK_{i,j} =K(\bx_i,\bx_j)$. 
\end{definition}
Kernel functions must be symmetric since inner products are always symmetric. In order to show that $K$ is a valid kernel, it is not always sufficient to show that a mapping $\bphi$ exists, but rather this is a nontrivial theoretical task. 
In practice, a real symmetric $N\times N$ matrix $\bK$, whose entries are $K(\bx_i,\bx_j)$ or simply $\bK_{i,j}$, is called \emph{positive definite}\index{positive definite} if for all $\alpha_1,\ldots,\alpha_N\in\mathbb{R}$, $\sum_{i,j=1}^N \alpha_i \alpha_j \bK_{i,j}\geq0$. A positive definite kernel produces a positive definite Gram matrix in the RKHS.
\begin{definition}\label{prop:kernelconstr}
Kernel matrices, which are constructed from a kernel corresponding to a strict inner product space $\mcalH$ are positive semidefinite. 
\end{definition}
This last property is easy to prove. Note that, by construction, we have $\bK_{i,j} = K(\bx_i,\bx_j)=\langle \bphi (\bx_i), \bphi (\bx_j)\rangle_{\mcalH}$, thus for any vector $\balpha \in\Real^N$:
\begin{equation}
\begin{split}
 \balpha^\top \bK  \balpha = & \sum_{i=1}^N\sum_{j=1}^N\alpha_i \bK_{i,j} \alpha_j = \sum_{i=1}^N\sum_{j=1}^N \alpha_i \langle \bphi (\bx_i), \bphi (\bx_j)\rangle_{\mcalH}\alpha_j \\
= & \bigg\langle\sum_i \alpha_i \bphi (\bx_i),\sum_j \alpha_j \bphi(\bx_j)\bigg\rangle_{\mcalH} = \bigg\|\sum_{i=1}^N \alpha_i \bphi (\bx_i)\bigg\|_{\mathcal H}^2\geq 0.
\end{split}
\end{equation}

Accordingly, any algorithm which operate on the data in such a way that it can be mathematically described in terms of dot products, can be used with any positive definite kernel by simply replacing $\langle \bphi(\bx),\bphi(\bx')\rangle_{\mcalH}$ with kernel evaluations $K(\bx,\bx')$, a technique known as \emph{kernelization} or \emph{kernel trick}~\cite{Scholkopf02}\index{kernel!kernel trick}. Moreover, for a positive definite kernel we do not need to know the explicit form of the feature map, but instead it is implicitly defined through the kernel calculation.

% ###############################################
\subsection{RKHS and Reproducing Property}\label{def_RKHS}
% ###############################################

In this section, we will define the notion of RKHS through the reproducing property. Then, we will see that a kernel function is a positive definite and symmetric function. It is also relevant to observe that the kernel fully generates the space, and that for a given kernel there is a unique RKHS; Conversely, every RKHS contains a single kernel. 

Let us assume a Hilbert space $\mathcal H$ where its elements are functions, provided with a dot product $\langle \cdot,\cdot \rangle $. We will denote $f(\cdot)$ as one element of the space, and $f(\bx)$ its value at a particular argument $\bx$. We will assume that arguments belong to a real or complex Euclidean space respectively, i.e. $\bx \in \mathbb{R}^N$ or $\bx \in \mathbb{C}^N$.

\begin{definition}{RKHS~\cite{Aronszajn50}.}
A Hilbert space $\mathcal{H}$ is said to be a RKHS if: (1) The elements of $\mathcal{H}$ are complex or real valued functions $f(\cdot)$ defined on any set of elements $\bx$; And (2) for every element $\bx$, $f(\cdot)$ is bounded.
\end{definition}
The name of these spaces come from the so-called {\em reproducing property}. Indeed, in an RKHS ${\mathcal{H}}$, there exists a function $K(\cdot,\cdot)$ such that 
\begin{equation}\label{RKHS_property}
f(\bx)=\langle f(\cdot),K(\cdot,\bx) \rangle , f \in \mathcal{H}
\end{equation}
by virtue of the Riesz Representation Theorem~\cite{RieNag55}. This function is called {\em kernel}.

\begin{property}
The kernel $K(\cdot,\cdot)$ is a positive definite and symmetric function.
\end{property}

{\proof Assume that  $f(\cdot)=K(\cdot,\bx)$ in Eq. \eqref{RKHS_property}. Hence, 
\begin{equation}
K(\bx,\bx')=\langle K(\cdot,\bx),K(\cdot,\bx') \rangle 
\end{equation}
Applying the complex conjugate operator $^\ast$ in the kernel and the dot product leads to
\begin{equation}
K^\ast(\bx,\bx')=(\langle K(\cdot,\bx),K(\cdot,\bx') \rangle )^\ast= \langle K(\cdot,\bx'),K(\cdot,\bx) \rangle =K(\bx',\bx),
\end{equation}
which proves that a kernel is symmetric. 
Besides, consider the series
\begin{equation}
\sum_{i=1}^N\alpha_i K(\cdot,\bx_i)
\end{equation} 
where $\alpha_i$ is any finite set of complex numbers. The norm of this series can be computed as
\begin{equation}
\bigg\|\sum_{i=1}^N\alpha_i K(\cdot,\bx_i)\bigg\|^2=\bigg\langle \sum_{i=1}^n\alpha_i K(\cdot,\bx_i),\sum_{j=1}^N\alpha_j, K(\cdot,\bx_j) \bigg\rangle.
\end{equation} 
By virtue of the reproducing property, $K(\bx_i,\bx_j)=\langle K(\cdot,\bx_i), K(\cdot,\bx_j) \rangle $, and by the linearity of the dot product, the above equation can be written as
\begin{equation}\label{kernel_norm}
\bigg\|\sum_{i=1}^N\alpha_i K(\cdot,\bx_i)\bigg\|^2=\sum_{i=1}^n \sum_{j=1}^n \alpha_i \alpha_j, K(\bx_i,\bx_j) \geq 0, 
\end{equation}
which proves that the kernel function is positive definite.}

{\property{The RKHS $\mathcal{H}$ with  a kernel $K$ is generated by $K(\cdot, \bx)$, where $\bx$ belongs to any set.}}
{\proof{It follows from the reproducing property that if $\langle f(\bx),K(\cdot,\bx) \rangle =0$, then, necessarily $f(\bx)=0$, hence all elements in $\mathcal{H}$ are generated by the kernel.}}

{\property{An RKHS contains a single reproducing kernel. Conversely, a reproducing kernel uniquely defines an RKHS.}}
{\proof{If we consider the linear space generated by $K$, we can define
\begin{equation}
\langle K(\cdot,\bx),K(\cdot,\bx') \rangle =K(\bx,\bx')
\end{equation}
Let us now consider two sets of scalars $\mu_i$ and $\lambda_j$, $1 \leq i,j \leq N$, then
\begin{equation}
\bigg\langle \sum_{i=1}^N\mu_i K(\cdot,\bx_i),\sum_{j=1}^N\lambda_j K(\cdot,\bx_j) \bigg\rangle =\sum_{i=1}^N\sum_{j=1}^N \mu_i  \lambda_j K(\bx_i,\bx_j)
\end{equation}
This expression satisfies the reproducing property and the requirements of dot product, as follows:
\begin{eqnarray}\nonumber
\begin{array}{lll}
K(\bx,\bx')&=&K^\ast(\bx',\bx')\\
\langle K(\cdot,\bx)+K(\cdot,\bx'),K(\cdot,\bx'') \rangle &=&\langle K(\cdot,\bx),K(\cdot,\bx') \rangle +\langle K(\cdot,\bx),K(\cdot,\bx'') \rangle \\
\langle \lambda K(\cdot,\bx),K(\cdot,\bx') \rangle &=&\lambda \langle K(\cdot,\bx),K(\cdot,\bx') \rangle \\
\langle K(\cdot,\bx),K(\cdot,\bx) \rangle &=&0 ~~~\text{if and only if}~~~K(\cdot,x)=0\\
\end{array} 
\end{eqnarray} 
The last requirement can be proven by using the Cauchy-Schwartz inequality,
\begin{equation}
\bigg\|\sum_{i=1}^N\lambda_i K(\cdot,\bx_i), K(\cdot,\bx) \rangle \bigg\|^2 \leq 
\sum_{i=1}^N\lambda_i K(\cdot,\bx_i),\sum_{j=1}^N\lambda_j K(\cdot,\bx_j) \rangle \langle K(\cdot,\bx),K(\cdot,\bx) \rangle 
\end{equation}
Hence, 
\begin{equation}
\bigg\langle \sum_{i=1}^N\lambda_i K(\cdot,\bx_i),\sum_{j=1}^N\lambda_j K(\cdot,\bx_j) \bigg\rangle =0
\end{equation}
implies 
\begin{equation}
\sum_{i=1}\lambda_i K(\bx,\bx_i)=0
\end{equation}
for every $\bx$. Therefore, $K$ is unique in $\mathcal{H}$ and it generates a unique RKHS.
}}

% ###############################
\subsection{Mercer's Theorem} 
% ###############################

Mercer's theorem is one of the most known results of the mathematician James Mercer (15 January 1883 -- 21 February 1932), and of fundamental importance in the context of kernel methods. Mercer's theorem is the key idea behind the so called {\em kernel trick}, which allows to solve a variety of nonlinear optimization problems through the construction of kernelized counterparts of linear algorithms. The Mercer's Theorem can be stated as follows.

Assume that $K(\cdot,\cdot)$ is a continuous kernel function satisfying the properties in Section \ref{def_RKHS}. Assume further that the kernel belongs to the family of square integrable functions. %Assume also the integral operator defined by 
%\begin{equation}
%L_Kf(\bx)=\int_{\mathcal X} K(\bx,\bx')f(\bx')d\mu(\bx'),
%\end{equation}
%where $\mu$ is any Borel measure. The eigenvalues $\phi_k$ of the operator form an orthonormal basis such that the corresponding eigenvalues $\lambda_k$ form a non-negative sequence. 

%\begin{theorem}[Mercer] The above defined kernel can be expressed as
%\begin{equation}
%K(\bx,\bx')=\sum_{k=1}^\infty \lambda_k \la \bphi(\bx),\bphi(\bx') \ra
%\end{equation}
%where the series converges uniformly for each pair $\bx, \bx'$. 
%\end{theorem}

 \begin{theorem}[Mercer's Theorem~\cite{Aizerman64}] Let $K(\bx, \bx')$ be a bivariate function fulfilling the Mercer condition, i.e., $\int_{\mathbb{R}^{N_r}\times \mathbb{R}^{N_r}} K(\bx, \bx') f(\bx)f(\bx')d\bx d\bx' \geq 0$ for any square integrable function $f(\bx)$. 
Then, there exists a RKHS $\mcalH$ and a mapping $\PHi(\cdot)$, such that $K(\bx, \bx') = \langle \bphi (\bx),\bphi(\bx') \rangle$.
\end{theorem}

We will now consider a set $D$ embedded in a space, typically we will use only $\mathbb{R}^d$ or $\mathbb{C}^d$. From the Mercer's Theorem, it follows that a mapping function $\bphi:\mathcal{D}\rightarrow \mathcal{H}$ can be expressed  as a (possibly infinite dimension) column vector:
\begin{equation}
\bphi(\bx)=\{\sqrt{\lambda_i}\bphi_i(\bx)\}_{i=1}^{\infty}.
\end{equation}
The dot product between two of these maps $\bphi(\bx_i)$ and $\bphi(\bx_2)$ is defined then as the kernel function of vectors $\bx$ and $\bx'$ as
\begin{equation}\label{eq:mercer_dot_prod}
\langle\bphi(\bx),\bphi(\bx')\rangle =\bphi(\bx)^\top\bphi(\bx') =\sum_{i=1}^\infty \lambda_i \bphi_i(\bx) \bphi_i(\bx')=K(\bx,\bx').
\end{equation}
The Mercer's Theorem shows that a mapping function into an RKHS and a dot product $K(\cdot,\cdot)$ exist if and only if $K(\cdot,\cdot)$ is a positive definite function. Hence, if a given function $\mathcal{D}\times\mathcal{D}\rightarrow \mathbb{R}$ (or $\mathbb{C}$) is proven to be positive definite, then it is the kernel of a given RKHS. 

{\example{Kernel function of band limited signals.}\label{example:sinc_kernel}
Consider the interval $\omega \in [-W, W]$, and the subspace of square integrable functions generated by complex exponentials as
\begin{equation}
\phi(t)=e^{\ii\omega t}.
\end{equation}
Since the dot product of square integrable functions is the integral of their product, the kernel function inside this RKHS is 
\begin{equation}\label{sinc_kernel}
\langle h(t_1),h(t_2) \rangle =\frac{1}{2W}\int_{-W}^W e^{\ii\omega t_1} e^{-\ii\omega t_2} d \omega = \frac{\sin(W(t_1 - t_2))}{W(t_1-t_2)}.
\end{equation}
This is then the kernel of the RKHS of signals that are band-limited to interval $W$. Moreover, the scalar dot product between functions is then
\begin{equation}
\langle f(\cdot),g(\cdot) \rangle =\int_{-W}^W F(\omega) G^\ast(\omega) d \omega,
\end{equation} 
where $F(\omega)$ and $G(\omega)$ are the FT of $f(t)$ and $g(t)$, respectively. Indeed, if we denote the FT operator as $\mathcal{F}()$ and use this dot product, the reproducing property 
\begin{equation}
f(t)=\langle f(\cdot),K(\cdot,t) \rangle =\int_{-W}^W F(\omega) \mathcal{F}^\ast(K(\cdot,t)) d \omega
\end{equation}
holds. From Eq.\eqref{sinc_kernel} it follows that $\mathcal{F}(K(\cdot,t))=e^{-\ii\omega t}$. Then   
\begin{equation}
f(t)=\langle f(\cdot),K(\cdot,t) \rangle =\int_{-W}^W F(\omega) e^{\ii\omega t} d \omega
\end{equation}
}

{\example{Second order polynomial kernel.} Kernel $K(\bx_i,\bx_j)=(1+\bx_i^\top\bx_j)^2$ is a particular case of $n$-th order polynomial kernels. Assuming that $\bx_i \in \mathbb{R}^2$, it is straightforward to find the mapping function $\phi:\mathbb{R}^2 \rightarrow \mathcal{H}$. If $\bx_i=\{x_i^{(1)}, x_i^{(2)}\}$, the dot product is 
\begin{equation}
K(\bx_i,\bx_j)=(1+\bx_i^\top\bx_j)^2=\left(1 + x_i^{(1)}x_j^{(1)} + x_i^{(2)}x_j^{(2)}\right)^2,
\end{equation}
which can be expanded as
\begin{equation*}
K(\bx_i,\bx_j) = 1 + \left(x_i^{(1)}x_j^{(1)}\right)^2 + \left(x_i^{(2)}x_j^{(2)}\right)^2 + 2x_i^{(1)}x_j^{(1)} + 2x_i^{(2)}x_j^{(2)} + 2x_i^{(1)}x_j^{(1)}x_i^{(2)}x_j^{(2)}.
\end{equation*}
By visual inspection, the corresponding mapping can be found to be
\begin{equation}
\bphi(\bx)=\left(  1,\left(x^{(1)}\right)^2,\left(x^{(2)}\right)^2,\sqrt{2}x^{(1)},\sqrt{2}x^{(2)},\sqrt{2}x^{(1)}x^{(2)} \right)^\top.
\end{equation}
Each element of this vector is an eigenfunction of this space. The corresponding eigenvectors are respectively $\lambda_1=\lambda_2=\lambda_3=1$, and $\lambda_4=\lambda_5=\lambda_6=\sqrt{2}$.
} % End of example


==> sections/notation.tex <==
\newcommand{\A}{\mathbf{A}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\D}{\mathbf{D}}

\newcommand{\K}{\mathbf{K}}
\newcommand{\II}{\mathbf{I}}
\newcommand{\KAD}{\K_{\mathrm{AD}}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\Q}{\mathbf{Q}}

\newcommand{\rota}[1]{\begin{sideways}#1\end{sideways}}

\newcommand{\ip}[2]{\langle {#1},\, {#2} \rangle}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\nlsum}{\sum\nolimits}

% Definitions.
% --------------------
\newcommand{\Real}{\mathbb R}
\newcommand{\Comp}{\mathbb C}

\def\x{{\mathbf x}}
\def\xk{{\mathbf x}^{(k)}}

\def\A{{\mathbf A}}
\def\B{{\mathbf B}}
\def\C{{\mathbf C}}
\def\LL{\boldsymbol{\Lambda}}
\def\Ak{{\mathbf A}_{(k)}}
\def\Bk{{\mathbf B}_{(k)}}
\def\I{{\mathbf I}}
\def\L{{\cal L}}
\def\U{{\mathbf U}}

\newcommand{\w}{{\mathbf w}}
\newcommand{\W}{{\mathbf W}}
\newcommand{\Z}{{\mathbf Z}}
\newcommand{\V}{{\mathbf V}}
\newcommand{\bb}{{\mathbf b}}
\newcommand{\e}{{\mathbf e}}
\newcommand{\uu}{{\mathbf u}}
\newcommand{\vv}{{\mathbf v}}
\newcommand{\bx}{{\mathbf x}}
\newcommand{\bw}{{\mathbf w}}
\newcommand{\bW}{{\mathbf W}}
\newcommand{\bv}{{\mathbf v}}
\newcommand{\bu}{{\mathbf u}}
\newcommand{\PP}{{\mathbf P}}
\newcommand{\Da}{{\mathbf D_a}}
\newcommand{\PHI}{\boldsymbol{\Phi}}
\newcommand{\PHi}{\boldsymbol{\phi}}
% Macros
\newcommand{\vect}[1]{{\boldsymbol{\mathbf{#1}}}} % vector
\newcommand{\mat}[1]{{\boldsymbol{\mathbf{#1}}}} % matrix
\newcommand{\y}{{\vect y}}
\newcommand{\f}{{\vect f}}
\newcommand{\g}{{\vect g}}
\newcommand{\s}{{\vect s}}
\newcommand{\mean}{{\vect \mu}}
\newcommand{\Sig}{{\mat \Sigma}}
\newcommand{\alp}{{\vect \alpha}}
\newcommand{\bet}{{\vect \beta}}
\newcommand{\kfs}{{\vect k}_{*}}
\newcommand{\kgs}{{\vect c}_{*}}
\newcommand{\kfss}{k_{**}}
\newcommand{\kgss}{c_{**}}
\newcommand{\bethat}{\overline{\vect \beta}}
\newcommand{\Kf}{{\mat K}_\vect{ff}}
\newcommand{\Kg}{{\mat K}_\vect{gg}}
\newcommand{\Kgu}{{\mat C}_{fv}}
\newcommand{\Ku}{{\mat C}_{vv}}
\newcommand{\Lam}{{\mat \Lambda}}
\newcommand{\Lamhat}{\overline{\mat \Lambda}}
\newcommand{\X}{{\mat X}}
\newcommand{\Y}{{\mat Y}}
\newcommand{\KL}[0]{\text{KL}}
\renewcommand{\d}[0]{\text{d}} 
\newcommand{\hyperf}{{\vect \theta}_k}
\newcommand{\hyperg}{{\vect \theta}_g}
\newcommand{\hyper}{{\vect \theta}}
\newcommand{\pmean}{{\vect \mu}}
\newcommand{\pcov}{{\mat \Sigma}}

\newcommand{\dataset}{{\cal D}}
\newcommand{\F}{{\cal F}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\maketilde}{\raisebox{0.4ex}{\tiny $\sim$}}

%------------------ Mine
\newcommand{\bigO}[0]{\mathcal{O}} 
\newcommand{\GP}[0]{\mathcal{GP}} 
\newcommand{\model}[0]{\mathcal{M}} 
%\newcommand{\R}[0]{\mathcal{R}} 
\newcommand{\Normal}[0]{\mathcal{N}} 
\newcommand{\Normnat}[0]{\mathcal{N}_\text{nat}} 
\renewcommand{\d}[0]{\text{d}} % derivative
\newcommand{\rank}[0]{\text{rank}} % trace
\newcommand{\rv}[1]{\ensuremath{\boldsymbol{#1}}} % random variable
\newcommand{\rvv}[1]{\ensuremath{\boldsymbol{{#1}}}} % random vector
\newcommand{\E}[0]{\mathbb{E}} 
\newcommand{\prob}{p}
\newcommand{\cov}[0]{\text{Cov}} 
\newcommand{\cut}[1]{} % cut out a part of the text
\newcommand{\Integer}[0]{\mathbb{Z}}  
\newcommand{\Natural}[0]{\mathbb{N}}  
\newcommand{\vectortwo}[2]{\left[\!\!\begin{array}{l}{#1}\\{#2}\end{array}\!\!\right]}
\newcommand{\vectorthree}[3]{\left[\!\!\begin{array}{l}{#1}\\{#2}\\{#3}\end{array}\!\!\right]}
\newcommand{\matrixfour}[4]{\left[\!\!\begin{array}{ll}  #1 & #2\\ #3 & #4\\ \end{array}\!\!\right]} 
\newcommand{\arrayfour}[4]{\left\{\begin{array}{ll}  #1 & #2\\ #3 & #4\\ \end{array}\right.}
\newcommand{\chol}{\operatorname{chol}}
\newcommand{\rot}{\operatorname{ro180}}
\newcommand{\tr}{\operatorname{trace}}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\erfc}{\operatorname{erfc}}
\newcommand{\diag}[0]{\operatorname{diag}} 
\newcommand{\blockdiag}[0]{\operatorname{bd}} 
\newcommand{\logit}[0]{\operatorname{logit}} 
\newcommand{\probit}{\operatorname{probit}}

\newcommand{\PSI}{\boldsymbol{\Psi}}
\newcommand{\PSi}{\boldsymbol{\psi}}
\newcommand{\aalpha}{\boldsymbol{\alpha}}
\newcommand{\BETA}{\boldsymbol{\beta}}
\newcommand{\h}{{\mathcal H}}
\newcommand{\HH}{{\mathbf K}}
\def\argmin{\mathop{\rm arg~min}}
\def\argmax{\mathop{\rm arg~max}}
\newcommand{\Intg}{\mathbb Z}
\DeclareMathOperator{\Lchula}{\mathcal{L}}
\DeclareMathOperator{\Rchula}{\mathbb{R}}
\DeclareMathOperator{\Ychula}{\mathcal{Y}}
\DeclareMathOperator{\abs}{abs}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\sinc}{sinc}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{definition}{Definition}[section]
%\newtheorem{property}{Property}[section]
%\newtheorem{property}[theorem]{Property}




==> styles/plos_one_macros.tex <==
% Text layout
\raggedright
\setlength{\parindent}{0.5cm}
\textwidth 5.25in 
\textheight 8.75in

% Bold the 'Figure #' in the caption and separate it from the title/caption with a period
% Captions will be left justified
\usepackage[aboveskip=1pt,labelfont=bf,labelsep=period,justification=raggedright,singlelinecheck=off]{caption}
\usepackage{color}
% \usepackage{natbib}

% Use the PLoS provided BiBTeX style
\bibliographystyle{styles/plos2015}

% Remove brackets from numbering in List of References
\makeatletter
\renewcommand{\@biblabel}[1]{\quad#1.}
\makeatother

% Leave date blank
\date{}

\usepackage[all]{xy}
\newcolumntype{x}[1]{>{\centering\arraybackslash\hspace{0pt}}p{#1}}

% Header and Footer with logo
\usepackage{lastpage,fancyhdr,graphicx}
\usepackage{epstopdf}
\pagestyle{myheadings}
\pagestyle{fancy}
\fancyhf{}
\lhead{\includegraphics[width=2.0in]{figures/logos/PLOS-submission.eps}}
\rfoot{\thepage/\pageref{LastPage}}
\renewcommand{\footrule}{\hrule height 2pt \vspace{2mm}}
\fancyheadoffset[L]{2.25in}
\fancyfootoffset[L]{2.25in}
\lfoot{\sf PLOS}

